Laplace HypoPINN: Physics-Informed Neural Network for hypocenter localization and its predictive uncertainty

Several techniques have been proposed over the years for automatic hypocenter localization. While those techniques have pros and cons that trade-off computational efficiency and the susceptibility of getting trapped in local minima, an alternate approach is needed that allows robust localization performance and holds the potential to make the elusive goal of real-time microseismic monitoring possible. Physics-informed neural networks (PINNs) have appeared on the scene as a flexible and versatile framework for solving partial differential equations (PDEs) along with the associated initial or boundary conditions. We develop HypoPINN -- a PINN-based inversion framework for hypocenter localization and introduce an approximate Bayesian framework for estimating its predictive uncertainties. This work focuses on predicting the hypocenter locations using HypoPINN and investigates the propagation of uncertainties from the random realizations of HypoPINN's weights and biases using the Laplace approximation. We train HypoPINN to obtain the optimized weights for predicting hypocenter location. Next, we approximate the covariance matrix at the optimized HypoPINN's weights for posterior sampling with the Laplace approximation. The posterior samples represent various realizations of HypoPINN's weights. Finally, we predict the locations of the hypocenter associated with those weights' realizations to investigate the uncertainty propagation that comes from those realisations. We demonstrate the features of this methodology through several numerical examples, including using the Otway velocity model based on the Otway project in Australia.

==> Sections/011_ImpactStatement.tex <==
\begin{IEEEImpStatement}
Determining microseismic hypocenter locations from traveltime observations is a classic inverse problem in geophysics. Over the years, several techniques have been proposed for automatic hypocenter localization. Yet, robust localization performance for real-time microseismic monitoring is far from trivial due to computational efficiency trade-offs and inversion challenges. Recent advances in deep learning have led to the development of our direct inversion framework for hypocenter localization based on physics-informed neural networks (PINNs). Our approach can recover relatively accurate prediction of the traveltime map and its associated hypocenter location even with a limited number of seismic observations. Furthermore, our approach is equipped with predictive uncertainty quantification, which is crucial for decision-making. This framework allows for computationally efficient and robust hypocenter localization that paves the way towards enabling real-time hypocenter localization for microseismic monitoring.
\end{IEEEImpStatement}

==> Sections/012_Keywords.tex <==
\begin{IEEEkeywords}
Deep learning, Approximate probabilistic inference, Simulation, Unsupervised learning, Neural networks
\end{IEEEkeywords}

==> Sections/08_Authors.tex <==
\begin{IEEEbiography}{Muhammad Izzatullah} received the bachelor’s degree in petroleum engineering from the Universiti Teknologi PETRONAS, Perak, Malaysia, in 2013, and the master’s degree in applied mathematics and computer science from the Novosibirsk State University, Novosibirsk, Russia, in 2017.

He is currently a PhD candidate with the Physical Sciences and Engineering Division, KAUST. His research interests broadly include the area of bayesian inference, waveform imaging, deep learning and deep generative modeling.
\end{IEEEbiography}

\begin{IEEEbiography}{Isa Eren Yildirim} received the bachelor’s degree in Geophysical engineering from Ankara University, Ankara, Turkey, in 2013, and the master’s degree in Earth Science and Engineering from KAUST. Then, he earned his second master's in applied mathematics from METU, Ankara, Turkey. 

He is currently a PhD candidate with the Physical Sciences and Engineering Division, KAUST. His research interests broadly include the area of Inverse Problems, Waveform imaging and Inversion, Deep learning.
\end{IEEEbiography}


\begin{IEEEbiography}{Umair Bin Waheed} received the Ph.D. degree in earth science and engineering from the King Abdullah University of Science and Technology, Thuwal, Saudi Arabia, in 2015.

He is an Assistant Professor of Geophysics with the King Fahd University of Petroleum and Minerals (KFUPM). Prior to joining KFUPM, he was a Post-Doctoral Fellow at the Department of Geosciences and a Fellow of Writing in Science and Engineering at the Princeton Writing Program, Princeton University. His research interests broadly include the area of computational geosciences.
\end{IEEEbiography}

\begin{IEEEbiography}{Tariq Alkhalifah} received the bachelor’s degree in geophysics from the King Fahd University of Petroleum and Minerals, Dhahran, Saudi Arabia, in 1988, and the master’s degree in geophysical engineering and the Ph.D. degree in geophysics from the Colorado School of Mines, Golden, CO, USA, in 1993 and 1997, respectively.

He joined the King Abdullah University of Science and Technology (KAUST), Thuwal, Saudi Arabia, in June 2009. Before he joined KAUST, he was a Research Professor and the Director of the Oil and Gas Research Institute, King Abdulaziz City for Science and Technology (KACST), Riyadh, Saudi Arabia. He held the positions of an Associate Research Professor, an Assistant Research Professor, and a Research Assistant at KACST. From 1996 to 1998, he was a Post-Doctoral Researcher for the Stanford Exploration Project at Stanford University, Stanford, CA, USA. He is currently a Professor with the Physical Sciences and Engineering Division, KAUST.

Dr. Alkhalifah is also a member of the Society of Exploration Geophysicists (SEG) and the European Association for Geoscientists and Engineers (EAGE). He received the J. Clarence Karcher Award from SEG, the Conrad Schlumberger Award from EAGE in 2003, and an Honorary Lecturer for the SEG in 2011.
\end{IEEEbiography}
